Microscopic Traffic Models, Accidents, and Insurance Losses

The paper develops a methodology to enable microscopic models of transportation systems to be accessible for a statistical study of traffic accidents. Our approach is intended to permit an understanding not only of historical losses, but also of incidents that may occur in altered, potential future systems. Through such a counterfactual analysis, it is possible, from an insurance, but also from an engineering perspective, to assess the impact of changes in the design of vehicles and transport systems in terms of their impact on road safety and functionality. Structurally, we characterize the total loss distribution approximatively as a mean-variance mixture. This also yields valuation procedures that can be used instead of Monte Carlo simulation. Specifically, we construct an implementation based on the open-source traffic simulator SUMO and illustrate the potential of the approach in counterfactual case studies.

==> Tables/Accidents/data01.tex <==
       1 &    0.011 &    0.012 &    0.030 &    0.033 &    0.082 &    0.098 &       51 &    0.015 &    0.016 &    0.047 &    0.048 &    0.117 &    0.178\\ 
       2 &    0.023 &    0.021 &    0.064 &    0.063 &    0.161 &    0.239 &       52 &    0.031 &    0.031 &    0.100 &    0.092 &    0.216 &    0.270\\ 
       3 &    0.020 &    0.019 &    0.068 &    0.056 &    0.153 &    0.196 &       53 &    0.033 &    0.029 &    0.091 &    0.079 &    0.228 &    0.345\\ 
       4 &    0.017 &    0.014 &    0.073 &    0.067 &    0.179 &    0.214 &       54 &    0.029 &    0.026 &    0.109 &    0.111 &    0.294 &    0.352\\ 
       5 &    0.027 &    0.027 &    0.069 &    0.058 &    0.156 &    0.183 &       55 &    0.035 &    0.030 &    0.132 &    0.130 &    0.284 &    0.373\\ 
       6 &    0.018 &    0.021 &    0.062 &    0.062 &    0.162 &    0.158 &       56 &    0.047 &    0.046 &    0.120 &    0.132 &    0.349 &    0.442\\ 
       7 &    0.018 &    0.018 &    0.049 &    0.061 &    0.135 &    0.158 &       57 &    0.049 &    0.045 &    0.133 &    0.129 &    0.305 &    0.484\\ 
       8 &    0.042 &    0.038 &    0.046 &    0.046 &    0.137 &    0.135 &       58 &    0.063 &    0.057 &    0.151 &    0.157 &    0.405 &    0.565\\ 
       9 &    0.019 &    0.017 &    0.041 &    0.042 &    0.119 &    0.118 &       59 &    0.059 &    0.058 &    0.155 &    0.167 &    0.455 &    0.568\\ 
      10 &    0.025 &    0.023 &    0.059 &    0.040 &    0.107 &    0.147 &       60 &    0.091 &    0.083 &    0.187 &    0.156 &    0.573 &    0.572\\ 
      11 &    0.023 &    0.023 &    0.059 &    0.048 &    0.213 &    0.160 &       61 &    0.063 &    0.068 &    0.196 &    0.206 &    0.515 &    0.638\\ 
      12 &    0.020 &    0.014 &    0.056 &    0.043 &    0.118 &    0.129 &       62 &    0.061 &    0.064 &    0.210 &    0.183 &    0.567 &    0.577\\ 
      13 &    0.030 &    0.029 &    0.076 &    0.043 &    0.180 &    0.155 &       63 &    0.056 &    0.074 &    0.203 &    0.227 &    0.616 &    0.585\\ 
      14 &    0.026 &    0.026 &    0.073 &    0.041 &    0.152 &    0.134 &       64 &    0.054 &    0.062 &    0.220 &    0.200 &    0.693 &    0.655\\ 
      15 &    0.028 &    0.037 &    0.055 &    0.045 &    0.169 &    0.182 &       65 &    0.071 &    0.071 &    0.262 &    0.213 &    0.705 &    0.627\\ 
      16 &    0.049 &    0.043 &    0.069 &    0.050 &    0.210 &    0.233 &       66 &    0.083 &    0.088 &    0.250 &    0.191 &    0.621 &    0.538\\ 
      17 &    0.024 &    0.027 &    0.061 &    0.060 &    0.184 &    0.216 &       67 &    0.084 &    0.077 &    0.233 &    0.213 &    0.656 &    0.696\\ 
      18 &    0.031 &    0.030 &    0.082 &    0.051 &    0.184 &    0.222 &       68 &    0.081 &    0.113 &    0.232 &    0.248 &    0.625 &    0.688\\ 
      19 &    0.031 &    0.031 &    0.076 &    0.069 &    0.200 &    0.217 &       69 &    0.085 &    0.088 &    0.251 &    0.207 &    0.653 &    0.490\\ 
      20 &    0.028 &    0.034 &    0.098 &    0.108 &    0.176 &    0.228 &       70 &    0.069 &    0.094 &    0.274 &    0.278 &    0.650 &    0.798\\ 
      21 &    0.033 &    0.041 &    0.064 &    0.089 &    0.191 &    0.251 &       71 &    0.077 &    0.086 &    0.239 &    0.199 &    0.745 &    0.558\\ 
      22 &    0.024 &    0.023 &    0.085 &    0.075 &    0.223 &    0.243 &       72 &    0.098 &    0.101 &    0.277 &    0.278 &    0.644 &    0.595\\ 
      23 &    0.031 &    0.024 &    0.065 &    0.076 &    0.221 &    0.237 &       73 &    0.066 &    0.115 &    0.217 &    0.226 &    0.637 &    0.610\\ 
      24 &    0.037 &    0.033 &    0.084 &    0.076 &    0.185 &    0.207 &       74 &    0.071 &    0.105 &    0.241 &    0.251 &    0.789 &    0.676\\ 
      25 &    0.024 &    0.030 &    0.071 &    0.065 &    0.226 &    0.206 &       75 &    0.090 &    0.083 &    0.209 &    0.251 &    0.803 &    0.638\\ 
      26 &    0.031 &    0.030 &    0.068 &    0.067 &    0.162 &    0.144 &       76 &    0.102 &    0.079 &    0.249 &    0.223 &    0.672 &    0.575\\ 
      27 &    0.034 &    0.033 &    0.071 &    0.064 &    0.196 &    0.227 &       77 &    0.082 &    0.103 &    0.177 &    0.256 &    0.627 &    0.579\\ 
      28 &    0.027 &    0.033 &    0.083 &    0.071 &    0.216 &    0.188 &       78 &    0.091 &    0.074 &    0.256 &    0.198 &    0.774 &    0.497\\ 
      29 &    0.031 &    0.030 &    0.071 &    0.075 &    0.179 &    0.317 &       79 &    0.101 &    0.095 &    0.286 &    0.227 &    0.793 &    0.676\\ 
      30 &    0.031 &    0.024 &    0.064 &    0.078 &    0.108 &    0.223 &       80 &    0.090 &    0.072 &    0.226 &    0.223 &    0.782 &    0.605\\ 
      31 &    0.032 &    0.026 &    0.076 &    0.067 &    0.142 &    0.245 &       81 &    0.099 &    0.077 &    0.236 &    0.244 &    0.891 &    0.622\\ 
      32 &    0.029 &    0.028 &    0.088 &    0.080 &    0.181 &    0.260 &       82 &    0.115 &    0.085 &    0.231 &    0.257 &    0.772 &    0.454\\ 
      33 &    0.032 &    0.025 &    0.073 &    0.073 &    0.208 &    0.246 &       83 &    0.116 &    0.048 &    0.252 &    0.269 &    0.713 &    0.820\\ 
      34 &    0.026 &    0.031 &    0.097 &    0.072 &    0.204 &    0.217 &       84 &    0.094 &    0.077 &    0.207 &    0.225 &    0.807 &    0.738\\ 
      35 &    0.027 &    0.032 &    0.075 &    0.095 &    0.200 &    0.228 &       85 &    0.084 &    0.117 &    0.208 &    0.274 &    0.687 &    0.909\\ 
      36 &    0.039 &    0.036 &    0.071 &    0.067 &    0.221 &    0.223 &       86 &    0.076 &    0.098 &    0.203 &    0.167 &    0.682 &    0.601\\ 
      37 &    0.033 &    0.042 &    0.072 &    0.068 &    0.165 &    0.209 &       87 &    0.101 &    0.133 &    0.216 &    0.237 &    0.866 &    0.622\\ 
      38 &    0.026 &    0.026 &    0.069 &    0.054 &    0.197 &    0.232 &       88 &    0.104 &    0.116 &    0.271 &    0.268 &    0.623 &    0.513\\ 
      39 &    0.029 &    0.038 &    0.069 &    0.077 &    0.197 &    0.232 &       89 &    0.123 &    0.099 &    0.220 &    0.238 &    0.664 &    0.507\\ 
      40 &    0.028 &    0.031 &    0.072 &    0.071 &    0.210 &    0.231 &       90 &    0.124 &    0.075 &    0.192 &    0.213 &    0.582 &    0.603\\ 
      41 &    0.039 &    0.037 &    0.085 &    0.118 &    0.157 &    0.242 &       91 &    0.109 &    0.074 &    0.199 &    0.260 &    0.595 &    0.617\\ 
      42 &    0.023 &    0.027 &    0.063 &    0.108 &    0.218 &    0.251 &       92 &    0.139 &    0.085 &    0.233 &    0.231 &    0.711 &    0.607\\ 
      43 &    0.034 &    0.035 &    0.075 &    0.135 &    0.196 &    0.200 &       93 &    0.122 &    0.084 &    0.233 &    0.203 &    0.773 &    0.680\\ 
      44 &    0.030 &    0.046 &    0.099 &    0.137 &    0.220 &    0.261 &       94 &    0.103 &    0.098 &    0.267 &    0.271 &    0.745 &    0.767\\ 
      45 &    0.029 &    0.038 &    0.107 &    0.098 &    0.193 &    0.228 &       95 &    0.100 &    0.098 &    0.286 &    0.232 &    0.751 &    0.679\\ 
      46 &    0.031 &    0.041 &    0.139 &    0.104 &    0.203 &    0.225 &       96 &    0.088 &    0.100 &    0.283 &    0.226 &    0.642 &    0.736\\ 
      47 &    0.033 &    0.035 &    0.101 &    0.109 &    0.198 &    0.196 &       97 &    0.101 &    0.111 &    0.283 &    0.310 &    0.647 &    0.802\\ 
      48 &    0.044 &    0.061 &    0.105 &    0.102 &    0.172 &    0.218 &       98 &    0.081 &    0.095 &    0.314 &    0.325 &    0.638 &    0.691\\ 
      49 &    0.021 &    0.032 &    0.114 &    0.135 &    0.175 &    0.175 &       99 &    0.110 &    0.102 &    0.329 &    0.308 &    0.696 &    0.703\\ 
      50 &    0.016 &    0.028 &    0.087 &    0.077 &    0.159 &    0.120 &      100 &    0.050 &    0.081 &    0.168 &    0.257 &    0.500 &    0.494\\ 


==> Tables/Accidents/data05.tex <==
       1 &    0.063 &    0.067 &    0.158 &    0.178 &    0.424 &    0.512 &       51 &    0.087 &    0.094 &    0.244 &    0.261 &    0.613 &    0.888\\ 
       2 &    0.128 &    0.126 &    0.287 &    0.312 &    0.926 &    1.236 &       52 &    0.165 &    0.172 &    0.512 &    0.509 &    1.277 &    1.791\\ 
       3 &    0.076 &    0.088 &    0.317 &    0.362 &    0.753 &    1.004 &       53 &    0.133 &    0.131 &    0.407 &    0.563 &    1.539 &    2.188\\ 
       4 &    0.070 &    0.063 &    0.340 &    0.343 &    0.957 &    1.228 &       54 &    0.149 &    0.141 &    0.526 &    0.650 &    1.617 &    1.980\\ 
       5 &    0.136 &    0.126 &    0.270 &    0.289 &    0.747 &    0.934 &       55 &    0.191 &    0.156 &    0.563 &    0.593 &    1.808 &    2.274\\ 
       6 &    0.078 &    0.102 &    0.264 &    0.284 &    0.971 &    0.930 &       56 &    0.218 &    0.231 &    0.522 &    0.639 &    1.959 &    2.337\\ 
       7 &    0.102 &    0.107 &    0.211 &    0.235 &    0.533 &    0.702 &       57 &    0.204 &    0.233 &    0.684 &    0.735 &    1.429 &    2.032\\ 
       8 &    0.119 &    0.122 &    0.225 &    0.194 &    0.561 &    0.705 &       58 &    0.223 &    0.173 &    0.561 &    0.652 &    1.922 &    2.272\\ 
       9 &    0.138 &    0.121 &    0.217 &    0.271 &    0.628 &    0.772 &       59 &    0.213 &    0.268 &    0.707 &    0.941 &    2.604 &    2.524\\ 
      10 &    0.130 &    0.123 &    0.299 &    0.251 &    0.606 &    0.999 &       60 &    0.240 &    0.214 &    0.784 &    0.858 &    2.953 &    2.798\\ 
      11 &    0.111 &    0.123 &    0.265 &    0.286 &    1.073 &    1.048 &       61 &    0.278 &    0.217 &    0.817 &    1.036 &    2.687 &    2.537\\ 
      12 &    0.122 &    0.133 &    0.211 &    0.294 &    1.050 &    0.819 &       62 &    0.272 &    0.349 &    0.898 &    0.958 &    2.813 &    3.100\\ 
      13 &    0.168 &    0.196 &    0.305 &    0.264 &    0.840 &    0.726 &       63 &    0.297 &    0.350 &    0.873 &    0.924 &    3.373 &    2.500\\ 
      14 &    0.158 &    0.124 &    0.205 &    0.214 &    0.980 &    0.789 &       64 &    0.404 &    0.346 &    0.840 &    1.063 &    2.989 &    2.898\\ 
      15 &    0.170 &    0.123 &    0.323 &    0.214 &    0.799 &    0.632 &       65 &    0.360 &    0.329 &    0.836 &    1.045 &    3.003 &    2.649\\ 
      16 &    0.148 &    0.134 &    0.352 &    0.243 &    1.009 &    0.621 &       66 &    0.319 &    0.384 &    0.963 &    1.025 &    2.705 &    3.167\\ 
      17 &    0.159 &    0.121 &    0.326 &    0.199 &    0.933 &    0.666 &       67 &    0.376 &    0.332 &    1.340 &    1.066 &    3.366 &    3.661\\ 
      18 &    0.206 &    0.164 &    0.365 &    0.315 &    1.006 &    0.945 &       68 &    0.411 &    0.292 &    1.028 &    1.117 &    3.318 &    3.275\\ 
      19 &    0.148 &    0.154 &    0.351 &    0.428 &    0.994 &    0.770 &       69 &    0.380 &    0.464 &    0.810 &    1.245 &    3.744 &    3.216\\ 
      20 &    0.180 &    0.110 &    0.360 &    0.362 &    0.912 &    0.929 &       70 &    0.513 &    0.483 &    1.062 &    1.217 &    2.970 &    3.024\\ 
      21 &    0.164 &    0.179 &    0.330 &    0.330 &    1.054 &    0.646 &       71 &    0.401 &    0.437 &    1.452 &    1.598 &    2.989 &    4.208\\ 
      22 &    0.189 &    0.139 &    0.490 &    0.409 &    1.001 &    0.918 &       72 &    0.391 &    0.401 &    1.032 &    1.269 &    2.794 &    3.274\\ 
      23 &    0.208 &    0.221 &    0.557 &    0.380 &    1.132 &    0.839 &       73 &    0.512 &    0.437 &    1.600 &    1.558 &    3.549 &    2.930\\ 
      24 &    0.158 &    0.178 &    0.429 &    0.278 &    0.755 &    0.672 &       74 &    0.336 &    0.520 &    1.319 &    1.372 &    2.913 &    3.336\\ 
      25 &    0.214 &    0.208 &    0.575 &    0.365 &    1.175 &    0.881 &       75 &    0.478 &    0.481 &    1.127 &    1.616 &    3.185 &    2.219\\ 
      26 &    0.233 &    0.224 &    0.507 &    0.420 &    0.798 &    0.777 &       76 &    0.410 &    0.561 &    1.271 &    1.367 &    2.591 &    2.516\\ 
      27 &    0.120 &    0.176 &    0.458 &    0.426 &    1.130 &    0.946 &       77 &    0.354 &    0.433 &    1.284 &    1.130 &    2.289 &    3.011\\ 
      28 &    0.263 &    0.199 &    0.549 &    0.317 &    1.305 &    1.108 &       78 &    0.551 &    0.416 &    1.220 &    0.890 &    2.830 &    2.836\\ 
      29 &    0.149 &    0.164 &    0.361 &    0.401 &    0.957 &    0.659 &       79 &    0.389 &    0.523 &    0.990 &    1.293 &    2.546 &    4.131\\ 
      30 &    0.158 &    0.190 &    0.353 &    0.337 &    0.960 &    0.763 &       80 &    0.357 &    0.552 &    1.213 &    1.126 &    2.879 &    3.642\\ 
      31 &    0.155 &    0.190 &    0.514 &    0.361 &    1.059 &    0.796 &       81 &    0.351 &    0.515 &    1.200 &    0.961 &    3.724 &    2.900\\ 
      32 &    0.154 &    0.215 &    0.683 &    0.385 &    0.611 &    0.711 &       82 &    0.390 &    0.428 &    1.186 &    1.323 &    3.836 &    3.237\\ 
      33 &    0.127 &    0.142 &    0.525 &    0.401 &    0.483 &    0.736 &       83 &    0.327 &    0.394 &    1.577 &    1.278 &    3.975 &    3.375\\ 
      34 &    0.100 &    0.172 &    0.571 &    0.384 &    0.873 &    0.810 &       84 &    0.371 &    0.427 &    1.633 &    1.169 &    3.878 &    3.206\\ 
      35 &    0.185 &    0.149 &    0.599 &    0.286 &    0.676 &    0.750 &       85 &    0.376 &    0.219 &    1.395 &    1.258 &    4.207 &    2.876\\ 
      36 &    0.177 &    0.206 &    0.521 &    0.416 &    0.980 &    0.681 &       86 &    0.433 &    0.352 &    1.616 &    0.914 &    3.997 &    3.670\\ 
      37 &    0.152 &    0.126 &    0.551 &    0.290 &    1.049 &    0.743 &       87 &    0.443 &    0.214 &    1.480 &    1.073 &    3.792 &    4.043\\ 
      38 &    0.160 &    0.174 &    0.446 &    0.349 &    0.922 &    0.694 &       88 &    0.403 &    0.253 &    1.307 &    0.911 &    2.677 &    4.091\\ 
      39 &    0.220 &    0.198 &    0.442 &    0.328 &    0.760 &    0.776 &       89 &    0.386 &    0.196 &    0.987 &    1.118 &    3.054 &    4.438\\ 
      40 &    0.139 &    0.150 &    0.444 &    0.333 &    0.937 &    0.730 &       90 &    0.374 &    0.408 &    1.080 &    1.298 &    3.068 &    3.832\\ 
      41 &    0.143 &    0.213 &    0.515 &    0.410 &    1.088 &    1.004 &       91 &    0.411 &    0.320 &    1.053 &    1.053 &    3.353 &    4.813\\ 
      42 &    0.135 &    0.147 &    0.624 &    0.482 &    0.961 &    0.744 &       92 &    0.374 &    0.481 &    1.105 &    1.343 &    3.303 &    5.189\\ 
      43 &    0.139 &    0.150 &    0.494 &    0.723 &    0.958 &    0.926 &       93 &    0.380 &    0.496 &    1.243 &    1.317 &    3.400 &    4.766\\ 
      44 &    0.169 &    0.162 &    0.441 &    0.539 &    0.922 &    0.887 &       94 &    0.408 &    0.450 &    1.172 &    1.382 &    4.417 &    5.476\\ 
      45 &    0.227 &    0.180 &    0.584 &    0.489 &    1.168 &    0.837 &       95 &    0.265 &    0.432 &    1.132 &    1.571 &    4.071 &    4.528\\ 
      46 &    0.122 &    0.127 &    0.481 &    0.320 &    1.455 &    0.679 &       96 &    0.274 &    0.440 &    1.029 &    1.450 &    3.714 &    4.625\\ 
      47 &    0.186 &    0.159 &    0.519 &    0.490 &    0.990 &    0.740 &       97 &    0.416 &    0.391 &    0.776 &    1.287 &    3.569 &    3.219\\ 
      48 &    0.253 &    0.164 &    0.460 &    0.447 &    0.852 &    0.716 &       98 &    0.276 &    0.584 &    1.393 &    1.487 &    3.659 &    3.135\\ 
      49 &    0.155 &    0.138 &    0.455 &    0.476 &    0.804 &    0.954 &       99 &    0.555 &    0.467 &    1.267 &    1.379 &    3.765 &    2.717\\ 
      50 &    0.077 &    0.066 &    0.301 &    0.292 &    0.563 &    0.238 &      100 &    0.145 &    0.157 &    0.598 &    0.986 &    1.552 &    1.396\\ 


==> Tables/Accidents/data09.tex <==
       1 &    0.210 &    0.248 &    0.404 &    0.437 &    0.914 &    0.990 &       51 &    0.260 &    0.298 &    0.535 &    0.667 &    1.451 &    1.711\\ 
       2 &    0.287 &    0.314 &    0.477 &    0.530 &    1.549 &    1.770 &       52 &    0.406 &    0.439 &    0.762 &    0.868 &    2.164 &    3.144\\ 
       3 &    0.163 &    0.166 &    0.544 &    0.583 &    1.633 &    1.527 &       53 &    0.376 &    0.382 &    0.754 &    0.957 &    2.538 &    3.412\\ 
       4 &    0.143 &    0.190 &    0.591 &    0.668 &    1.814 &    1.801 &       54 &    0.301 &    0.322 &    0.998 &    1.153 &    2.934 &    3.744\\ 
       5 &    0.226 &    0.246 &    0.471 &    0.613 &    1.449 &    1.896 &       55 &    0.259 &    0.450 &    0.784 &    1.321 &    2.952 &    4.352\\ 
       6 &    0.309 &    0.285 &    0.406 &    0.539 &    1.652 &    1.492 &       56 &    0.423 &    0.486 &    1.059 &    1.127 &    3.487 &    3.803\\ 
       7 &    0.242 &    0.257 &    0.493 &    0.508 &    1.580 &    1.517 &       57 &    0.535 &    0.482 &    0.872 &    1.300 &    3.307 &    4.277\\ 
       8 &    0.251 &    0.224 &    0.393 &    0.393 &    1.250 &    1.218 &       58 &    0.424 &    0.446 &    1.226 &    1.110 &    3.606 &    4.653\\ 
       9 &    0.263 &    0.270 &    0.410 &    0.402 &    1.139 &    1.274 &       59 &    0.371 &    0.434 &    1.061 &    1.428 &    5.064 &    5.213\\ 
      10 &    0.277 &    0.283 &    0.485 &    0.390 &    1.280 &    1.149 &       60 &    0.596 &    0.531 &    1.130 &    1.416 &    4.542 &    4.558\\ 
      11 &    0.251 &    0.250 &    0.690 &    0.485 &    2.027 &    1.528 &       61 &    0.371 &    0.478 &    1.172 &    1.469 &    5.310 &    6.026\\ 
      12 &    0.232 &    0.396 &    0.643 &    0.438 &    1.789 &    1.191 &       62 &    0.478 &    0.453 &    1.431 &    1.583 &    5.881 &    6.296\\ 
      13 &    0.244 &    0.287 &    0.553 &    0.474 &    2.114 &    1.350 &       63 &    0.493 &    0.500 &    1.762 &    1.832 &    6.149 &    5.773\\ 
      14 &    0.296 &    0.327 &    0.668 &    0.440 &    2.016 &    1.140 &       64 &    0.471 &    0.522 &    1.392 &    2.168 &    6.499 &    6.421\\ 
      15 &    0.402 &    0.387 &    0.497 &    0.365 &    1.706 &    1.208 &       65 &    0.518 &    0.481 &    1.697 &    2.105 &    6.589 &    5.943\\ 
      16 &    0.327 &    0.313 &    0.867 &    0.469 &    1.834 &    1.105 &       66 &    0.590 &    0.608 &    1.666 &    1.725 &    5.099 &    6.180\\ 
      17 &    0.380 &    0.271 &    0.613 &    0.467 &    2.007 &    1.234 &       67 &    0.720 &    0.572 &    1.969 &    1.838 &    5.481 &    5.559\\ 
      18 &    0.215 &    0.270 &    0.641 &    0.434 &    1.632 &    1.260 &       68 &    0.709 &    0.439 &    1.681 &    2.332 &    5.331 &    7.396\\ 
      19 &    0.227 &    0.264 &    0.581 &    0.386 &    2.032 &    1.187 &       69 &    0.620 &    0.506 &    1.937 &    1.692 &    5.138 &    6.560\\ 
      20 &    0.416 &    0.365 &    0.657 &    0.496 &    2.012 &    1.342 &       70 &    0.559 &    0.600 &    1.447 &    2.172 &    5.150 &    6.256\\ 
      21 &    0.220 &    0.320 &    0.572 &    0.402 &    2.080 &    1.366 &       71 &    0.648 &    0.593 &    1.776 &    2.041 &    6.764 &    7.774\\ 
      22 &    0.260 &    0.286 &    0.695 &    0.531 &    2.215 &    1.675 &       72 &    0.744 &    0.612 &    2.249 &    1.709 &    6.999 &    5.912\\ 
      23 &    0.271 &    0.342 &    0.895 &    0.738 &    2.302 &    1.458 &       73 &    0.738 &    0.831 &    1.805 &    1.920 &    6.551 &    6.062\\ 
      24 &    0.280 &    0.400 &    0.620 &    0.715 &    1.869 &    1.230 &       74 &    0.669 &    0.615 &    2.074 &    2.042 &    6.351 &    5.598\\ 
      25 &    0.239 &    0.350 &    0.662 &    0.699 &    1.993 &    1.370 &       75 &    0.574 &    0.621 &    1.762 &    2.243 &    4.736 &    7.480\\ 
      26 &    0.260 &    0.496 &    0.725 &    0.436 &    1.753 &    1.155 &       76 &    0.588 &    0.614 &    1.858 &    2.150 &    6.260 &    7.337\\ 
      27 &    0.283 &    0.332 &    0.565 &    0.540 &    2.034 &    1.317 &       77 &    0.529 &    0.476 &    2.130 &    1.893 &    5.756 &    5.461\\ 
      28 &    0.260 &    0.324 &    0.898 &    0.529 &    1.974 &    1.049 &       78 &    0.507 &    0.560 &    1.881 &    2.278 &    4.603 &    5.212\\ 
      29 &    0.495 &    0.294 &    0.662 &    0.570 &    1.873 &    1.331 &       79 &    0.479 &    0.633 &    1.965 &    2.036 &    4.229 &    5.506\\ 
      30 &    0.350 &    0.289 &    0.963 &    0.433 &    2.010 &    1.215 &       80 &    0.491 &    0.754 &    1.414 &    2.478 &    4.102 &    6.615\\ 
      31 &    0.398 &    0.268 &    0.574 &    0.632 &    1.641 &    1.359 &       81 &    0.366 &    0.692 &    2.418 &    2.221 &    4.906 &    4.359\\ 
      32 &    0.321 &    0.314 &    0.438 &    0.847 &    2.325 &    1.564 &       82 &    0.585 &    0.739 &    2.081 &    2.322 &    5.959 &    6.304\\ 
      33 &    0.338 &    0.272 &    0.428 &    1.309 &    1.897 &    1.637 &       83 &    0.592 &    0.627 &    2.665 &    1.675 &    4.790 &    6.161\\ 
      34 &    0.369 &    0.270 &    0.286 &    0.623 &    2.006 &    1.366 &       84 &    0.680 &    0.673 &    1.780 &    2.044 &    5.923 &    6.777\\ 
      35 &    0.466 &    0.456 &    0.467 &    0.887 &    1.964 &    1.387 &       85 &    0.619 &    0.513 &    1.458 &    1.512 &    7.145 &    6.888\\ 
      36 &    0.371 &    0.293 &    0.754 &    0.640 &    2.163 &    1.318 &       86 &    0.414 &    0.614 &    1.707 &    1.731 &    6.458 &    7.630\\ 
      37 &    0.411 &    0.233 &    0.684 &    0.681 &    1.902 &    1.182 &       87 &    0.618 &    0.575 &    1.713 &    1.955 &    7.100 &    5.358\\ 
      38 &    0.398 &    0.281 &    0.678 &    0.743 &    1.838 &    1.249 &       88 &    0.462 &    0.490 &    2.347 &    1.834 &    6.681 &    7.801\\ 
      39 &    0.396 &    0.269 &    0.558 &    0.528 &    1.883 &    1.513 &       89 &    0.416 &    0.680 &    2.425 &    2.981 &    6.499 &    4.090\\ 
      40 &    0.524 &    0.375 &    0.741 &    0.751 &    1.979 &    1.452 &       90 &    0.499 &    0.629 &    1.539 &    3.613 &    5.169 &    5.765\\ 
      41 &    0.362 &    0.284 &    0.772 &    0.667 &    2.446 &    1.071 &       91 &    0.648 &    0.644 &    1.859 &    3.113 &    4.926 &    4.817\\ 
      42 &    0.441 &    0.310 &    0.857 &    0.757 &    1.996 &    1.653 &       92 &    0.458 &    0.657 &    2.884 &    3.438 &    6.093 &    4.222\\ 
      43 &    0.457 &    0.303 &    0.919 &    0.975 &    1.944 &    1.471 &       93 &    0.530 &    0.700 &    3.324 &    2.417 &    5.460 &    5.895\\ 
      44 &    0.463 &    0.461 &    0.829 &    0.640 &    1.966 &    1.383 &       94 &    0.829 &    0.780 &    3.284 &    2.561 &    5.435 &    5.650\\ 
      45 &    0.666 &    0.340 &    0.591 &    0.702 &    2.016 &    1.261 &       95 &    0.446 &    0.766 &    2.211 &    2.420 &    5.502 &    6.146\\ 
      46 &    0.683 &    0.596 &    0.826 &    0.617 &    2.132 &    1.203 &       96 &    0.822 &    0.641 &    2.095 &    1.994 &    4.905 &    6.230\\ 
      47 &    0.690 &    0.650 &    0.511 &    0.777 &    1.819 &    1.264 &       97 &    0.708 &    0.504 &    2.410 &    1.986 &    5.911 &    6.273\\ 
      48 &    0.543 &    0.338 &    0.676 &    0.584 &    1.874 &    1.120 &       98 &    0.425 &    0.428 &    1.741 &    2.001 &    5.398 &    6.954\\ 
      49 &    0.449 &    0.319 &    0.523 &    0.722 &    1.743 &    1.264 &       99 &    0.533 &    0.512 &    2.714 &    2.325 &    6.597 &    7.637\\ 
      50 &    0.245 &    0.164 &    0.488 &    0.466 &    1.586 &    0.810 &      100 &    0.213 &    0.234 &    1.043 &    1.066 &    4.294 &    4.861\\ 


==> Tables/TableNormal/table052aNonUnif.tex <==
\begin{table} 
\centering 
\scalebox{0.7}{ 
\begin{threeparttable} 
\caption{Statistical Functionals of Normalized $L$ for Non-Uniform Accident Occurrence with $\rho^\Phi=0.5$ and $\zeta^{2a}$.} 
\begin{tabular}{rrrrrrrrrrrrrr} \toprule 
& \multicolumn{6}{c}{Binomial Model}  & \quad\quad & \multicolumn{6}{c}{Poisson Model}   \\ \midrule 
& \multicolumn{3}{c}{Gamma}  & \multicolumn{3}{c}{Log-Normal} & & \multicolumn{3}{c}{Gamma}  & \multicolumn{3}{c}{Log-Normal}  \\ \midrule 
& $c_v=0.5$ & $c_v=1.0$ & $c_v=2.0$  & $c_v=0.5$ & $c_v=1.0$ & $c_v=2.0$ & & $c_v=0.5$ & $c_v=1.0$ & $c_v=2.0$  &  $c_v=0.5$ & $c_v=1.0$ & $c_v=2.0$  \\     \toprule 
&\multicolumn{13}{c}{\textbf{Non-Uniform Accident Occurrence}}  \\ 
$\mathbb{E}(L)$ &     93.5 &     93.1 &     93.5 &     93.7 &     93.4 &     93.8 & &     93.6 &     93.8 &     93.8 &     93.6 &     93.6 &     93.6 \\ 
$\mathrm{Var}(L)$&    562.5 &    870.7 &   2199.0 &    569.1 &    867.6 &   2158.7 & &    559.7 &    879.1 &   2183.6 &    559.8 &    873.1 &   2177.8 \\ 
$\varsigma_L$ &    0.333 &    0.561 &    0.993 &    0.377 &    0.660 &    2.152 & &    0.299 &    0.522 &    1.045 &    0.417 &    0.711 &    2.155 \\ 
$\mathrm{VaR}_{0.9}(L)$  &    125.1 &    131.5 &    156.1 &    125.2 &    132.9 &    149.7 & &    124.5 &    133.0 &    155.5 &    124.3 &    132.0 &    148.7 \\ 
$\mathrm{ES}_{0.9}(L)$ &    138.2 &    150.4 &    191.6 &    138.8 &    151.6 &    194.4 & &    137.7 &    151.4 &    191.6 &    138.5 &    152.0 &    193.6 \\ 
$\mathrm{VaR}_{0.95}(L)$ &    134.9 &    146.5 &    182.0 &    135.6 &    146.3 &    177.6 & &    134.7 &    146.8 &    182.5 &    134.5 &    145.9 &    174.4 \\ 
$\mathrm{ES}_{0.95}(L)$ &    146.3 &    162.8 &    215.0 &    147.6 &    164.3 &    227.5 & &    146.1 &    163.8 &    215.8 &    148.0 &    165.7 &    226.9 \\ 
$\mathrm{VaR}_{0.99}(L)$ &    153.3 &    171.3 &    237.0 &    154.6 &    174.4 &    250.6 & &    153.6 &    174.6 &    238.7 &    156.8 &    176.4 &    256.7 \\ 
$\mathrm{ES}_{0.99}(L)$ &    163.3 &    189.0 &    266.1 &    166.5 &    191.7 &    321.4 & &    163.4 &    188.8 &    269.3 &    168.6 &    196.4 &    325.4 \\ 
\bottomrule 
\end{tabular} 
\begin{tablenotes} 
\small 
\item The statistical functionals of the normalized total loss are approximated using $10,000$ independent samples of $L$. Total losses are normalized by $100$ expected insured vehicles.
\end{tablenotes} 
\end{threeparttable} 
}
\label{tab1}

\end{table}


==> Tables/TableTotal/table052a.tex <==
\begin{table} 
\centering 
\scalebox{0.7}{ 
\begin{threeparttable} 
\caption{Statistical Functionals of $L$ for $\rho^\Phi=0.5$ and $\zeta^{2a}$.} 
\begin{tabular}{rrrrrrrrrrrrrr} \toprule 
& \multicolumn{6}{c}{Binomial Model}  & \quad\quad & \multicolumn{6}{c}{Poisson Model}   \\ \midrule 
& \multicolumn{3}{c}{Gamma}  & \multicolumn{3}{c}{Log-Normal} & & \multicolumn{3}{c}{Gamma}  & \multicolumn{3}{c}{Log-Normal}  \\ \midrule 
& $c_v=0.5$ & $c_v=1.0$ & $c_v=2.0$  & $c_v=0.5$ & $c_v=1.0$ & $c_v=2.0$ & & $c_v=0.5$ & $c_v=1.0$ & $c_v=2.0$  &  $c_v=0.5$ & $c_v=1.0$ & $c_v=2.0$  \\     \toprule 
 \\ 
&\multicolumn{13}{c}{\textbf{Uniform Accident Occurrence}}  \\ 
$\mathbb{E}(L)$  &   6074.1 &   6060.6 &   6057.3 &   6062.5 &   6071.7 &   6062.5 & &   6066.6 &   6081.9 &   6049.3 &   6082.6 &   6070.7 &   6079.3 \\ 
$\mathrm{Var}(L)$ & 1090361.3 & 1517008.9 & 2989042.5 & 1099229.5 & 1466766.0 & 3154753.0 & & 1084491.1 & 1493958.5 & 3021932.0 & 1112695.1 & 1464801.0 & 3003597.9 \\ 
$\varsigma_L$ &    0.198 &    0.309 &    0.466 &    0.187 &    0.336 &    1.361 & &    0.194 &    0.272 &    0.509 &    0.220 &    0.342 &    1.035 \\ 
$\mathrm{VaR}_{0.9}(L)$ &   7461.5 &   7700.1 &   8349.7 &   7463.1 &   7670.1 &   8310.1 & &   7449.9 &   7702.2 &   8402.7 &   7488.8 &   7658.5 &   8291.5 \\ 
$\mathrm{ES}_{0.9}(L)$ &   7959.6 &   8345.3 &   9362.0 &   7944.3 &   8335.4 &   9654.3 & &   7943.3 &   8345.5 &   9418.3 &   8000.3 &   8328.4 &   9569.1 \\ 
$\mathrm{VaR}_{0.95}(L)$ &   7845.2 &   8173.1 &   9099.5 &   7814.5 &   8164.5 &   9153.4 & &   7830.2 &   8212.8 &   9181.0 &   7875.9 &   8146.9 &   9162.1 \\ 
$\mathrm{ES}_{0.95}(L)$  &   8278.5 &   8779.1 &  10033.9 &   8263.9 &   8764.4 &  10610.2 & &   8268.1 &   8758.7 &  10082.2 &   8332.4 &   8777.0 &  10466.3 \\ 
$\mathrm{VaR}_{0.99}(L)$ &   8551.2 &   9184.5 &  10689.5 &   8518.7 &   9115.0 &  11381.5 & &   8571.2 &   9144.8 &  10612.5 &   8621.4 &   9166.7 &  11181.0 \\ 
$\mathrm{ES}_{0.99}(L)$ &   8890.3 &   9675.5 &  11515.2 &   8891.9 &   9659.7 &  13317.7 & &   8876.7 &   9519.7 &  11415.2 &   8932.9 &   9687.3 &  12778.9 \\   
&\multicolumn{13}{c}{\textbf{Non-Uniform Accident Occurrence}}  \\ 
$\mathbb{E}(L)$ &   1315.3 &   1322.3 &   1326.0 &   1322.7 &   1321.7 &   1324.5 & &   1317.3 &   1310.7 &   1321.2 &   1319.6 &   1313.1 &   1317.2 \\ 
$\mathrm{Var}(L)$& 168470.4 & 245780.8 & 583773.9 & 166082.8 & 243388.7 & 587217.4 & & 164276.7 & 235282.1 & 558258.2 & 165179.6 & 242009.7 & 537609.2 \\ 
$\varsigma_L$ &    0.431 &    0.676 &    1.164 &    0.430 &    0.705 &    2.822 & &    0.423 &    0.588 &    1.147 &    0.439 &    0.684 &    1.955 \\ 
$\mathrm{VaR}_{0.9}(L)$ &   1867.4 &   1989.7 &   2347.5 &   1866.8 &   1979.8 &   2232.2 & &   1861.8 &   1964.7 &   2308.0 &   1866.4 &   1979.8 &   2227.4 \\  
$\mathrm{ES}_{0.9}(L)$ &   2102.3 &   2305.4 &   2953.9 &   2101.1 &   2302.4 &   2945.4 & &   2091.5 &   2263.6 &   2893.3 &   2097.1 &   2298.3 &   2910.6 \\  
$\mathrm{VaR}_{0.95}(L)$ &   2045.8 &   2210.9 &   2786.2 &   2041.8 &   2211.1 &   2671.0 & &   2032.5 &   2177.7 &   2719.4 &   2048.1 &   2230.6 &   2663.9 \\ 
$\mathrm{ES}_{0.95}(L)$ &   2255.8 &   2518.5 &   3358.9 &   2256.5 &   2516.8 &   3475.0 & &   2242.9 &   2463.8 &   3284.4 &   2248.2 &   2507.1 &   3396.2 \\ 
$\mathrm{VaR}_{0.99}(L)$ &   2386.4 &   2699.8 &   3719.7 &   2406.8 &   2681.7 &   3894.6 & &   2376.1 &   2623.4 &   3547.6 &   2384.1 &   2673.4 &   3740.7 \\  
$\mathrm{ES}_{0.99}(L)$ &   2556.9 &   2996.5 &   4271.0 &   2560.1 &   2985.6 &   5121.0 & &   2530.3 &   2883.0 &   4118.5 &   2553.7 &   2908.6 &   4797.2 \\ 
\bottomrule 
\end{tabular} 
\begin{tablenotes} 
\small 
\item The statistical functionals of the total loss are approximated using $10,000$ independent samples of $L$. 
\end{tablenotes} 
\end{threeparttable} 
}
\label{tab1}

\end{table}


==> Tables/TableTotal/table052aNonUnif.tex <==
\begin{table} 
\centering 
\scalebox{0.7}{ 
\begin{threeparttable} 
\caption{Statistical Functionals of $L$ for $\rho^\Phi=0.5$ and $\zeta^{2a}$.} 
\begin{tabular}{rrrrrrr} \toprule 
& \multicolumn{6}{c}{Binomial Model}    \\ \midrule 
& \multicolumn{3}{c}{Gamma}  & \multicolumn{3}{c}{Log-Normal}   \\ \midrule 
& $c_v=0.5$ & $c_v=1.0$ & $c_v=2.0$  & $c_v=0.5$ & $c_v=1.0$ & $c_v=2.0$   \\     \toprule 
 \\ 
$\mathbb{E}(L)$ &   1315.3 &   1322.3 &   1326.0 &   1322.7 &   1321.7 &   1324.5  \\ 
$\mathrm{Var}(L)$& 168470.4 & 245780.8 & 583773.9 & 166082.8 & 243388.7 & 587217.4  \\ 
$\varsigma_L$ &    0.431 &    0.676 &    1.164 &    0.430 &    0.705 &    2.822 \\ 
$\mathrm{VaR}_{0.9}(L)$ &   1867.4 &   1989.7 &   2347.5 &   1866.8 &   1979.8 &   2232.2 \\  
$\mathrm{ES}_{0.9}(L)$ &   2102.3 &   2305.4 &   2953.9 &   2101.1 &   2302.4 &   2945.4  \\  
$\mathrm{VaR}_{0.95}(L)$ &   2045.8 &   2210.9 &   2786.2 &   2041.8 &   2211.1 &   2671.0  \\ 
$\mathrm{ES}_{0.95}(L)$ &   2255.8 &   2518.5 &   3358.9 &   2256.5 &   2516.8 &   3475.0  \\ 
$\mathrm{VaR}_{0.99}(L)$ &   2386.4 &   2699.8 &   3719.7 &   2406.8 &   2681.7 &   3894.6  \\  
$\mathrm{ES}_{0.99}(L)$ &   2556.9 &   2996.5 &   4271.0 &   2560.1 &   2985.6 &   5121.0  \\ 
\bottomrule 
\end{tabular} 
\begin{tablenotes} 
\small 
\item The statistical functionals of the total loss are approximated using $10,000$ independent samples of $L$. 
\end{tablenotes} 
\end{threeparttable} 
}
\label{tab1}

\end{table}

